Explaining Bias in Deep Face Recognition via Image Characteristics

In this paper, we propose a novel explanatory framework aimed to provide a better understanding of how face recognition models perform as the underlying data characteristics (protected attributes: gender, ethnicity, age; non-protected attributes: facial hair, makeup, accessories, face orientation and occlusion, image distortion, emotions) on which they are tested change. With our framework, we evaluate ten state-of-the-art face recognition models, comparing their fairness in terms of security and usability on two data sets, involving six groups based on gender and ethnicity. We then analyze the impact of image characteristics on models performance. Our results show that trends appearing in a single-attribute analysis disappear or reverse when multi-attribute groups are considered, and that performance disparities are also related to non-protected attributes. Source code: https://cutt.ly/2XwRLiA.

==> ijcb2022/tables/RQ1.1/DiveFace/RQ1.1_AttentionNetNPCFace.tex <==
\begin{subtable}{1.\linewidth}{
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rra|rra}
\hline
{} & \multicolumn{3}{l}{\textbf{FAR}} & \multicolumn{3}{l}{\textbf{FRR}} \\
 &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} \\
\hline
\emph{Asian}     &  0.048 &  0.043 &  0.046 &  0.045 &  0.042 &  0.043 \\
\emph{Black}     &  0.047 &  0.045 &  0.046 &  \textbf{0.050} &  0.041 &  0.045 \\
\emph{Caucasian} &  \textbf{0.051} &  0.049 &  0.050 &  0.048 &  0.036 &  0.042 \\
\rowcolor{boxgrey}
\emph{$A \cup B \cup C$}    &  0.049 &  0.045 &  0.047 &  0.048 &  0.040 &  0.044 \\
\hline
\end{tabular}}}
\vspace{-2mm}
\caption{AttentionNet + NPCFace}
\vspace{2mm}
\end{subtable}

==> ijcb2022/tables/RQ1.1/DiveFace/RQ1.1_HRNetNPCFace.tex <==
\begin{subtable}{1.\linewidth}{
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rra|rra}
\hline
{} & \multicolumn{3}{l}{\textbf{FAR}} & \multicolumn{3}{l}{\textbf{FRR}} \\
 &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} \\
\hline
\emph{Asian}     &  \textbf{0.055} &  0.048 &  0.051 &  0.041 &  0.043 &  0.042 \\
\emph{Black}     &  0.044 &  0.041 &  0.043 &  \textbf{0.056} &  0.048 &  0.052 \\
\emph{Caucasian} &  0.053 &  0.051 &  0.052 &  0.047 &  0.041 &  0.044 \\
\rowcolor{boxgrey}
\emph{$A \cup B \cup C$}      &  0.051 &  0.046 &  0.049 &  0.048 &  0.044 &  0.046 \\
\hline
\end{tabular}}}
\vspace{-2mm}
\caption{HRNet + NPCFace}
\vspace{2mm}
\end{subtable}

==> ijcb2022/tables/RQ1.1/DiveFace/RQ1.1_RepVGGNPCFace.tex <==
\begin{subtable}{1.\linewidth}{
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rra|rra}
\hline
{} & \multicolumn{3}{l}{\textbf{FAR}} & \multicolumn{3}{l}{\textbf{FRR}} \\
 &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} \\
\hline
\emph{Asian}     &  \textbf{0.080} &  0.067 &  0.073 &  0.067 &  0.063 &  0.065 \\
\emph{Black}     &  0.065 &  0.057 &  0.061 &  0.084 &  \textbf{0.087} &  0.085 \\
\emph{Caucasian} &  0.079 &  0.077 &  0.078 &  0.061 &  0.055 &  0.058 \\
\rowcolor{boxgrey}
\emph{$A \cup B \cup C$}     &  0.075 &  0.067 &  0.071 &  0.071 &  0.068 &  0.069 \\
\hline
\end{tabular}}}
\vspace{-2mm}
\caption{RepVGG + NPCFace}
\vspace{2mm}
\end{subtable}

==> ijcb2022/tables/RQ1.1/DiveFace/RQ1.1_ResNeStNPCFace.tex <==
\begin{subtable}{1.\linewidth}{
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rra|rra}
\hline
{} & \multicolumn{3}{l}{\textbf{FAR}} & \multicolumn{3}{l}{\textbf{FRR}} \\
 &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} \\
\hline
\emph{Asian}     &  \textbf{0.077} &  0.068 &  0.072 &  0.058 &  0.069 &  0.064 \\
\emph{Black}     &  0.057 &  0.054 &  0.055 &  0.064 &  0.071 &  0.065 \\
\emph{Caucasian} &  0.076 &  0.069 &  0.073 &  \textbf{0.078} &  0.055 &  0.067 \\
\rowcolor{boxgrey}
\emph{$A \cup B \cup C$}    &  0.070 &  0.064 &  0.067 &  0.067 &  0.065 &  0.066 \\
\hline
\end{tabular}}}
\vspace{-2mm}
\caption{ResNeSt + NPCFace}
\vspace{-2mm}
\end{subtable}

==> ijcb2022/tables/RQ1.1/DiveFace/RQ1.1_ResNet152NPCFace.tex <==
\begin{subtable}{1.\linewidth}{
\vspace{2mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rra|rra}
\hline
{} & \multicolumn{3}{l}{\textbf{FAR}} & \multicolumn{3}{l}{\textbf{FRR}} \\
 &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} \\
\hline
\emph{Asian}     &  \textbf{0.034} &  0.029 &  0.032 &  0.024 &  0.029 &  0.026 \\
\emph{Black}     &  0.028 &  0.022 &  0.025 &  \textbf{0.035} &  0.027 &  0.031 \\
\emph{Caucasian} &  0.034 &  0.029 &  0.032 &  0.028 &  0.021 &  0.025 \\
\rowcolor{boxgrey}
\emph{$A \cup B \cup C$}      &  0.032 &  0.027 &  0.029 &  0.029 &  0.026 &  0.027 \\
\hline
\end{tabular}}}
\vspace{-2mm}
\caption{ResNet152 + NPCFace}
\vspace{2mm}
\end{subtable}

==> ijcb2022/tables/RQ1.1/VGG/RQ1.1_AttentionNetNPCFace.tex <==
\begin{subtable}{.62\textwidth}{
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rra|rra}
\hline
{} & \multicolumn{3}{l}{\textbf{FAR}} & \multicolumn{3}{l}{\textbf{FRR}} \\
 &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} \\
\hline
\emph{Asian}     &  0.293 &  0.117 &  0.205 &  \textbf{0.300} &  0.200 &  0.250 \\
\emph{Black}     &  0.180 &  0.172 &  0.176 &  0.200 &  0.200 &  0.200 \\
\emph{Caucasian} &  \textbf{0.330} &  0.224 &  0.277 &  0.133 &  0.200 &  0.167 \\
\rowcolor{boxgrey}
\emph{$A \cup B \cup C$}    &  0.268 &  0.171 &  0.219 &  0.211 &  0.2 &  0.206 \\
\hline
\end{tabular}}}
\vspace{-2mm}
\caption{AttentionNet + NPCFace}
\vspace{2mm}
\end{subtable}

==> ijcb2022/tables/RQ1.1/VGG/RQ1.1_HRNetNPCFace.tex <==
\begin{subtable}{.62\textwidth}{
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rra|rra}
\hline
{} & \multicolumn{3}{l}{\textbf{FAR}} & \multicolumn{3}{l}{\textbf{FRR}} \\
 &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} \\
\hline
\emph{Asian}     &  0.320 &  0.130 &  0.225 &  \textbf{0.367} &  0.133 &  0.250 \\
\emph{Black}     &  0.172 &  0.162 &  0.167 &  0.240 &  0.275 &  0.258 \\
\emph{Caucasian} &  \textbf{0.333} &  0.252 &  0.293 &  0.133 &  0.120 &  0.127 \\
\rowcolor{boxgrey}
\emph{$A \cup B \cup C$}      &  0.275 &  0.182 &  0.228 &  0.247 &  0.176 &  0.211 \\
\hline
\end{tabular}}}
\vspace{-2mm}
\caption{HRNet + NPCFace}
\vspace{2mm}
\end{subtable}

==> ijcb2022/tables/RQ1.1/VGG/RQ1.1_RepVGGNPCFace.tex <==
\begin{subtable}{.62\textwidth}{
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rra|rra}
\hline
{} & \multicolumn{3}{l}{\textbf{FAR}} & \multicolumn{3}{l}{\textbf{FRR}} \\
 &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} \\
\hline
\emph{Asian}     &  0.333 &  0.163 &  0.248 &  \textbf{0.367} &  0.133 &  0.250 \\
\emph{Black}     &  0.228 &  0.205 &  0.216 &  0.280 &  0.225 &  0.252 \\
\emph{Caucasian} &  \textbf{0.417} &  0.284 &  0.350 &  0.167 &  0.360 &  0.263 \\
\rowcolor{boxgrey}
\emph{$A \cup B \cup C$}     &  0.326 &  0.217 &  0.272 &  0.271 &  0.239 &  0.255 \\
\hline
\end{tabular}}}
\vspace{-2mm}
\caption{RepVGG + NPCFace}
\vspace{2mm}
\end{subtable}

==> ijcb2022/tables/RQ1.1/VGG/RQ1.1_ResNeStNPCFace.tex <==
\begin{subtable}{.62\textwidth}{
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rra|rra}
\hline
{} & \multicolumn{3}{l}{\textbf{FAR}} & \multicolumn{3}{l}{\textbf{FRR}} \\
 &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} \\
\hline
\emph{Asian}     &  0.336 &  0.153 &  0.245 &  0.333 &  0.233 &  0.283 \\
\emph{Black}     &  0.260 &  0.195 &  0.227 &  \textbf{0.360} &  0.250 &  0.305 \\
\emph{Caucasian} &  \textbf{0.413} &  0.252 &  0.332 &  0.133 &  0.240 &  0.186 \\
\rowcolor{boxgrey}
\emph{$A \cup B \cup C$}    &  0.336 &  0.200 &  0.268 &  0.275 &  0.241 &  0.258 \\
\hline
\end{tabular}}}
\vspace{-2mm}
\caption{ResNeSt + NPCFace}
\vspace{-2mm}
\end{subtable}

==> ijcb2022/tables/RQ1.1/VGG/RQ1.1_ResNet152NPCFace.tex <==
\begin{subtable}{.62\textwidth}{
\vspace{2mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rra|rra}
\hline
{} & \multicolumn{3}{l}{\textbf{FAR}} & \multicolumn{3}{l}{\textbf{FRR}} \\
 &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} &    \emph{Woman} &      \emph{Man} &       \emph{$W \cup M$} \\
\hline
\emph{Asian}     &  \textbf{0.227} &  0.163 &  0.195 &  0.233 &  0.133 &  0.183 \\
\emph{Black}     &  0.128 &  0.138 &  0.133 &  \textbf{0.240} &  0.175 &  0.208 \\
\emph{Caucasian} &  0.237 &  0.248 &  0.242 &  0.133 &  0.080 &  0.107 \\
\rowcolor{boxgrey}
\emph{$A \cup B \cup C$}      &  0.197 &  0.183 &  0.190 &  0.202 &  0.129 &  0.166 \\
\hline
\end{tabular}}}
\vspace{-2mm}
\caption{ResNet152 + NPCFace}
\vspace{2mm}
\end{subtable}

==> ijcb2022/tables/backbones_info_CR.tex <==
\begin{table}[t!]
\begin{center}
\resizebox{1.00\linewidth}{!}{
\begin{tabular}{rr|rrr|rrr|r}
\hline
\multicolumn{2}{c}{\textbf{Face Models}$^{1, 2}$}                           & \multicolumn{3}{l}{\textbf{DiveFace}} & \multicolumn{3}{l}{\textbf{VGG-Face2}} & \multicolumn{1}{l}{}                                         \\
Backbone     & Head    & EER  & 1\%$^3$ & 0.1\%$^3$ & EER  & 1\%$^3$ & 0.1\%$^3$ & \#Params \\
\hline
ResNet152    & MagFace & 0.04 & 0.10      & 0.22        & 0.21 & 0.62      & 0.77        & 80M     \\
\ul{ResNet152}    & \ul{NPCFace} & \textbf{0.03} & 0.05      & 0.12        & \textbf{0.19} & 0.52      & 0.73        & 80M     \\
HRNet        & MagFace & 0.20 & 0.56      & 0.69        & 0.33 & 0.90      & 0.96        & 79M     \\
\ul{HRNet}        & \ul{NPCFace} & \textbf{0.05} & 0.11      & 0.24        & \textbf{0.21} & 0.60      & 0.81        & 79M     \\
AttentionNet & MagFace & 0.06 & 0.16      & 0.32        & 0.23 & 0.71      & 0.88        & 108M    \\
\ul{AttentionNet} & \ul{NPCFace} & \textbf{0.04} & 0.11      & 0.25        & \textbf{0.22} & 0.65      & 0.82        & 108M    \\
RepVGG       & MagFace & 0.07 & 0.28      & 0.44        & 0.28 & 0.80      & 0.93        & 116M    \\
\ul{RepVGG}       & \ul{NPCFace} & \textbf{0.07} & 0.18      & 0.34        & \textbf{0.28} & 0.74      & 0.91        & 116M    \\
ResNeSt      & MagFace & 0.10 & 0.85      & 0.88        & 0.26 & 0.77      & 0.88        & 86M     \\
\ul{ResNeSt}      & \ul{NPCFace} & \textbf{0.07} & 0.17      & 0.31        & \textbf{0.27} & 0.71      & 0.89        & 86M       \\
\hline
\multicolumn{9}{l}{$^1$ Due to space constraints, our study focused on the \ul{best setting} per backbone.} \tabularnewline
\multicolumn{9}{l}{$^2$ Models have an avg. size of 377.49$\pm$60 megabytes.} \tabularnewline
\multicolumn{9}{l}{$^3$ Reported values refer to FRRs w.r.t. the specified FAR percentage threshold.} \tabularnewline
\tabularnewline
\end{tabular}}
\end{center}
\vspace{-6mm}
\caption{Statistics on the considered face encoders.}
\label{tab:backbones}
\end{table}

==> ijcb2022/tables/datasets_info.tex <==
\begin{table*}[t!]
\label{table:3}
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|rrr|rr|rr}
\hline
\textbf{Data Set Name}  & \textbf{Part}  & \textbf{\# Images} & \textbf{\# Users} & \textbf{Avg. Images/User} & \textbf{Avg. Images/Group} & \textbf{\# Groups}                   & \textbf{\% Minority}                   & \textbf{\% Majority}                       \\
\hline
DiveFace     & Training       & 111,503  & 19,196 & 6 $\pm$ 8           & 18,584 $\pm$ 2,968       & 6  & 49.07 (Male); 29.23 (Black)   & 50.92 (Female); 39.96 (Caucasian) \\
DiveFace     & Test       & 28,236  & 4,804 & 6 $\pm$ 11           & 4,706 $\pm$ 875       & 6  & 48.94 (Female); 27.72 (Black)   & 51.05 (Male); 39.91 (Caucasian) \\
VGG-Face2$^1$  & Test & 134,766 & 449  & 300 $\pm$ 108       & 22,461 $\pm$ 26,694         & 6  & 41.95 (Female); 4.71 (Black) & 58.04 (Male); 82.02 (Caucasian) \\ 
\hline
\multicolumn{8}{l}{$^1$ Our experiments did not include models trained on \texttt{VGG-Face2}. For training, we used only \texttt{DiveFace}, which ensures a good representation of all demographic groups.} \tabularnewline
\end{tabular}
}
\end{center}
\vspace{-6mm}
\caption{Relevant descriptive information of the two data sets considered in our study.}
\label{tab:data}
\end{table*}

==> ijcb2022/tables/related_works_v3.tex <==
\begin{table*}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|lllll|llllll|lllll}
\hline
\multicolumn{2}{l}{\textbf{Study Information}}               & \multicolumn{5}{|l}{\textbf{Sensitive Attribute(s)}$^1$} & \multicolumn{6}{|l|}{\textbf{Face Data Set(s)}} & \multicolumn{5}{|l}{\textbf{Evaluation Metric(s)$^2$}}          \\
\textit{Authors}                                             & \textit{Type}       & \textit{G}    & \textit{E}    & \textit{A}    & \textit{S}   & \textit{I}   & \textit{VGG} & \textit{IJB} & \textit{LFW} & \textit{BUPT} & \textit{RFW} & \textit{Other(s)}                  & \textit{FPR/FNR} & \textit{ROC} & \textit{AUC} & \textit{Accuracy} & \textit{Other(s)} \\
\hline
Terhorst, P et al. \cite{comp_demo}                 & Analysis   & X    & X    &      & X   &     &     &           &     &      &     & MAAD                         & X       &     &     &          & EER, MAD      \\
Majumdar et al \cite{unravelling}                   & Analysis   & X    & X    &      &     &     &     &           &     &      &     & MORPH, MUCT                  &         &     &     &          & DoB      \\
Albiero et al. \cite{genderineq}                    & Analysis   & X    & X    &      &     &     &     &           &     &      &     & MORPH                        & X       & X   &     &          &          \\
Albiero \& Bowyer \cite{sexist}                      & Analysis   & X    &      &      &     &     &     &           &     &      &     & MORPH, Notre Dame            & X       &     &     &          &          \\
Dooley et al. \cite{robust_face_det}                & Analysis   & X    & X    & X    &     &     &     &           &     &      &     & O-Images, MIAP, CCD, UtkFace &         &     &     &          & mrCE     \\
Hupont \& Fernandez \cite{demogpairs}               & Analysis   &      & X    &      &     &     & X   & X         & X   &      &     & CWF                          & X       &     &     &          &          \\
Popescu et al. \cite{popescu2021face}               & Analysis   & X    & X    & X    &     &     &     & X         & X   &      &     &                              &         &     &     & X        &          \\
Rosenberg et al. \cite{FaceRecObf}                  & Analysis   & X    & X    &      &     &     & X   &           & X   &      &     &                              & X       &     & X   &          &          \\
\hline
Kortylewskiet et al. \cite{kortylewski2019synthetic}& Mitigation &      &      &      &     & X   &     & X         & X   &      &     & CMU                          & X       &     &     &          &          \\
Gwilliam et al. \cite{mitigate_racial}              & Mitigation & X    & X    &      &     &     &     &           &     & X    & X   &                              &         &     &     & X        &          \\
Wang et al. \cite{9512390}                          & Mitigation &      & X    & X    & X   &     &     &           &     & X    &     &                              &         & X   &     & X        &          \\
Alasadi et al. \cite{FairnessFaceMatch}             & Mitigation &      & X    &      &     &     &     &           &     &      &     & Celeb-A/UMD                  & X       &     &     & X        &          \\
Wang et al. \cite{Wang2019RacialFI}                 & Mitigation &      & X    &      & X   &     &     & X         &     &      & X   &                              & X       &     &     & X        &          \\
Gong et al. \cite{groupadaptivemitig}               & Mitigation &      & X    &      &     &     &     & X         & X   & X    & X   &                              & X       &     &     & X        &          \\
Rodriguez et al. \cite{9025435}                     & Mitigation & X    &      &      &     &     & X   &           &     &      &     &                              & X       & X   & X   &          &          \\
Terhorst, P et al. \cite{comparisonlevelmitig}      & Mitigation &      & X    &      &     &     &     &           & X   &      &     &                              & X       & X   & X   &          & EER      \\
\hline
\multicolumn{18}{l}{$^1$ G : Gender, E : Ethnicity, A: Age, S: Soft Attribute(s), I : Identity.} \tabularnewline
\multicolumn{18}{l}{$^2$ FPR/FNR : False Positive/Negative Rate, AUC : Area under the ROC Curve, EER : Equal Error Rate, DoB : Degree of Bias, mrCE : mean relative Corruption Error, MAD : Mean Absolute Deviation.} \tabularnewline
\end{tabular}

}
\vspace{-4mm}
\caption{Summary table about research on exploration and mitigation of unfairness in face recognition.}
\label{tab:prior-work}
\end{table*}
